PuppetDroid: A User-Centric UI Exerciser for Automatic Dynamic Analysis of Similar Android Applications

Popularity and complexity of malicious mobile applications are rising, making their analysis difficult and labor intensive. Mobile application analysis is indeed inherently different from desktop application analysis: In the latter, the interaction of the user (i.e., victim) is crucial for the malware to correctly expose all its malicious behaviors. We propose a novel approach to analyze (malicious) mobile applications. The goal is to exercise the user interface (UI) of an Android application to effectively trigger malicious behaviors, automatically. Our key intuition is to record and reproduce the UI interactions of a potential victim of the malware, so as to stimulate the relevant behaviors during dynamic analysis. To make our approach scale, we automatically re-execute the recorded UI interactions on apps that are similar to the original ones. These characteristics make our system orthogonal and complementary to current dynamic analysis and UI-exercising approaches. We developed our approach and experimentally shown that our stimulation allows to reach a higher code coverage than automatic UI exercisers, so to unveil interesting malicious behaviors that are not exposed when using other approaches. Our approach is also suitable for crowdsourcing scenarios, which would push further the collection of new stimulation traces. This can potentially change the way we conduct dynamic analysis of (mobile) applications, from fully automatic only, to user-centric and collaborative too.

==> approach.tex <==
\section{Proposed approach}
\label{sec:proposed-approach}

The main limitation of dynamic analysis is its inability to obtain a high level
of code coverage: dynamic analysis, indeed, can examine the actions performed
in an execution path only if that path is actually explored. This problem is
particularly serious for malware analysis: a piece of malware that is not
properly exercised may not expose its malicious behavior, misleading analysts
to label it as benign. Exercising mobile applications in a proper way, however,
is not a trivial problem, because of the use of highly-interactive UI to best
leverage the capabilities of modern touchscreens, making automatic exercising
of their interfaces harder, with respect to conventional PCs scenario.

Current dynamic solutions integrate their analysis engines with automatic
exercising and stimulation techniques. These techniques can be roughly divided
in two main branches: those that leverage stress-test tools, like
Monkey~\cite{androidDoc_monkey}, and those that use program analysis, like
SmartDroid~\cite{smartdroid} and ActEVE~\cite{anand2012automated}. Stress-test
tools rely on pseudo-random generation of UI input events. This approach is
simple to implement, but rather ineffective, since randomly stimulating UI
elements displayed on the screen can hardly reproduce the typical usage of
users (except, maybe, for the cat's paw typing case). On the other end,
approaches like DynoDroid~\cite{dynodroid} and SmartDroid~\cite{smartdroid}
leverage static analysis to reconstruct the semantic of UI elements on the
screen, to find execution paths that expose malicious behaviors. However,
static analysis is greatly hindered by obfuscated code or dynamic payloads,
two techniques widely used by modern malware. 

In this paper we describe a solution for the problem of application exercising
for malware analysis purposes. In particular, we propose a new approach to
exercise the UI of an Android application that changes the way malware analysis
experiments are currently conducted, and effectively stimulate potentially
malicious behaviors. The key intuition behind our solution is to leverage
human-driven exercising. As a matter of fact, human users are much more
effective at exercising an application than automatic tools because they
understand the semantic of elements displayed on the screen and exercise the
application accordingly. Unfortunately, however, the number of human resources
required to exercise the huge amount of application published every day would
be unreasonably large. To downsize this blocking resource requirement, we
leverage a second key observation, derived by security reports by AV
vendors~\cite{eset2012,trendmicro2012} \FIXME{and research papers (cite)} that
report a quite common practice among mobile malware authors: repackaging of
existent malware samples inside different legitimate apps, to obtain slightly
different variants able to avoid AV detection
techniques~\FIXME{citation}. Furthermore, to gain higher infection rates,
miscreants usually repackage their malware inside well-known, non-free apps
that are then released free of charge to be more appealing for unaware users
(\FIXME{vero? citation needed}). \FIXME{Qua secondo me va spiegato un po'
  meglio il repackaging, perch\'e non \`e immediatamente evidente il rapporto
  tra repackaging e similarity}. We leverage this phenomenon to make our
approach scale: in fact, our idea is to record a trace of the human-driven UI
stimulation, that we name \emph{stimulation trace}, performed during a test and
leverage code similarity to automatically re-execute this trace on applications
similar to one originally tested by the user. In this way, if at least one user
in our system succeeds in manually stimulating a malicious behavior in a
malware, it is quite likely that by re-using the same \strace on similar
applications, we can stimulate similar malicious behaviors.

On top of our observations, we design and implement an Android sandboxed
environment able to support both \textit{manual application testing}, to
collect new \straces, and \textit{automatic application exercising}, which
cleverly leverages previously recorded UI \straces.

\FIXME{Mettere in we did: Furthermore, we also want to experimentally verify if
  manual exercising allows to better stimulate malicious behaviors than
  automatic exercising techniques. Finally, we want to experimentally validate
  our approach and demonstrate that it brings an original contribution to the
  state of the art, allowing to overcome current limitations in application
  exercising for malware analysis purposes.}

% \begin{itemize}
% \item Problem we want to face: poor code coverage of automatic dynamic analysis approaches
%   \begin{itemize}
%   \item pseudo-random generation of UI events (monkey) hardly reproduces the typical usage of a human user
%   \item combination of static analysis and automatic UI exercisers: ineffective in case of obfuscated code or dynamic payloads
%   \end{itemize}
% \item Our key intuitions:
%   \begin{itemize}
%   \item leverage human-driven exercising: they understand the semantic of elements displayed on the screen and can exercise the application accordingly
%   \item leverage app similarity (repackaged malware phenomenon): re-execute previously recorded human-driven stimulation on similar applications (introduce the concept of stimulation trace)
%   \end{itemize}
% \item Our approach: propose two ways to perform dynamic analysis
%   \begin{itemize}
%   \item Manual Test: the user directly interacts with the application and executes the test leveraging the sandboxed environment we provide
%   \item Automatic Test: the user leverages previously recorded UI stimulation traces performed on similar samples to automatically exercise the application
%   \end{itemize}
% \item Logical workflow of the approach illustrated with user interaction with PuppetDroid(e.g., Fig:~\ref{fig:approach_diagram})
% \end{itemize}

% \begin{figure}[!t]
% \centering
% \includegraphics[width=2.5in]{approach_diagram}
% \caption{Activity diagram of user interaction with PuppetDroid system.}
% \label{fig:approach_diagram}
% \end{figure}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 

